Superconvergent Non-Polynomial Approximations

In this paper, we introduce a superconvergent approximation method that employs radial basis functions (RBFs) in the numerical solution of conservation laws. The use of RBFs for interpolation and approximation is a well developed area of research. Of particular interest in this work is the development of high order finite volume (FV) weighted essentially non-oscillatory (WENO) methods, which utilize RBF approximations to obtain required data at cell interfaces. Superconvergence is addressed through an analysis of the truncation error, resulting in expressions for the shape parameters that lead to improvements in the accuracy of the approximations. This study seeks to address the practical elements of the approach, including the evaluations of shape parameters as well as hybrid implementation. To highlight the effectiveness of the non-polynomial basis, in shock-capturing, the proposed methods are applied to one-dimensional hyperbolic and weakly hyperbolic systems of conservation laws and compared with several well-known FV WENO schemes in the literature. In the case of the non-smooth, weakly hyperbolic test problem, notable improvements are observed in predicting the location and height of the finite time blowup. The convergence results demonstrate that the proposed schemes attain notable improvements in accuracy, as indicated by the analysis of the reconstructions. We also include a discussion regarding extensions to higher dimensional problems, along with convergence results for a nonlinear scalar problem.

==> ch3superconvergentRBF.tex <==
\section{Supercovergent RBF schemes}
\label{sec: Superconvergent schemes}

In this section, we derive the expressions for optimal shape, or tension, parameters for RBF interpolation. We provide analyses in section \ref{subsec: Parameter} using two reconstruction methods: a direct approach using integrals and a second approach that utilizes a primitive function. Here, we choose the shape parameter $\lambda$, for a given RBF $\phi$, so that it maximizes the convergence order of the interpolation. 

\subsection{Optimal Shape Parameters for RBFs}\label{subsec: Parameter}

In \cite{HKYY}, the authors introduced a WENO scheme based on the space of exponential polynomials. Later, in the work \cite{HKYY-2}, they improved the order of accuracy of their schemes by exploiting the control parameter $\lambda \in \RR$ or $i\RR$ for exponential basis functions of the form $e^{\lambda x}$. We adopt a similar strategy in this work with the difference being the choice of the basis. Here, the basis functions consist of infinitely smooth RBFs $\phi$ (see Table \ref{tab:rbf}) rather than exponential polynomials. We present detailed analyses using the Gaussian RBF 
\begin{align}\label{rbf:gauss}
    \phi(x)=e^{-\lambda^2 x^2}, \quad \lambda\in \RR \text{ or } i\RR,
\end{align}
in the case of $N = 2$, using two different approaches. For each approach, we provide analytical expressions for the optimal shape parameters, which allow the schemes to achieve superconvergence on a fixed reconstruction stencil. 

% \begin{comment}
% We consider a system of conservation laws $ \partial_t u + \nabla \cdot f(u)=0 $ where $u$ is a vector of conserved quantities and $f$ is a vector of vector valued of flux functions. Here we focus on the one-dimensional spatial case:
% \begin{align}\label{eq:claw}
% \partial_t u + \partial_x f(u)=0.
% \end{align}
% We restrict our considerations to uniformly distributed spatial grids with grid cells $I_i:=[x_{i-1/2},x_{i+1/2}]$ and grid spacing $\Delta x= x_{i+1/2}-x_{i-1/2}$ for all $i$. A finite volume method for the equation \eqref{eq:claw} can be written in the semi-discrete form
% \begin{align}
% \frac{d}{dt}u_i = - \frac{1}{\Delta x} (\hat{F}_{i+1/2} - \hat{F}_{i-1/2}).
% \end{align}
% Given the cell averages $\bar{u}_i(x)$ of a function $u(x)$ for each cell $I_i$, we construct the RBF reconstruction from cell averages.
% \end{comment}

% \begin{comment}
% Here we use the approximation form \eqref{rbf_interpol} in the system \eqref{rbf_lin} with $m=0$ for simplicity:
% \begin{align*}%\label{rbf_fv_interpol}
% Au_X(x):= \sum_{k=1}^{N} \alpha_k  \phi(x-x_k)
% \end{align*}
% satisfying:
% \begin{align*}
%     \frac{1}{\Delta x}\int_{I_i}Au_X(\xi)d\xi = \bar{u}_i, \quad \forall i=1,\cdots, N,
% \end{align*}
% i.e., we need to solve the system
% \begin{align*}
%     \sum_{k=1}^{N} \alpha_k \frac{1}{\Delta x}\int_{I_i} \phi(\xi-x_k) d\xi = \bar{u}_i, \quad \forall i=1,\cdots, N.
% \end{align*}
% \end{comment}

\subsubsection{Direct Computation with Integrals}
\label{subsubsec: Direct with integrals}

% In this section, we demonstrate how the choice of the right shape parameter facilitates RBF interpolation achieving higher order on a fixed number of points than the equivalent traditional polynomial interpolation.  Further, we give an analytic expression for the form of the shape parameter that lets the method achieve high than expected order. 

Recall that the RBF approximation is given by
\begin{align}\label{rbf_app2}
Au(x):= \sum_{k=1}^{2} \alpha_k  \phi(x-x_{j+k-1})= \alpha_1  \phi(x-x_{j}) +\alpha_2  \phi(x-x_{j+1}).
\end{align}
The goal is to form a high order approximation using the form \eqref{rbf_app2}, which preserves each of the cell averages. In other words, the approximation should satisfy the integral constraint
\begin{align}\label{rbf_app2_cond}
    \frac{1}{\Delta x}\int_{I_i} Au(\xi) d\xi =\bar{u}_i, \quad i=j,{\ }j+1.
    %\frac{1}{\Delta x}\int_{x_{i-1/2}}^{x_{i+1/2}} Au(\xi) d\xi =\bar{u}_i, \quad i=j,j+1.
\end{align}
Using the RBF $\phi(x)$ defined in \eqref{rbf:gauss}, it follows that the integrals of $\phi$ can be evaluated analytically, which resulting in a solvable linear system. Once the solution is determined, the final approximation at the cell boundary $x_{j+\frac{1}{2}}$ is given by
\begin{align*}
    Au(x_{j+\frac{1}{2}})=\frac{ 2\lambda \Delta x\exp(-\frac{\lambda^2\Delta x^2}{4}) }
    { \sqrt{\pi} \big( \erf(\frac{\lambda \Delta x}{2}) + \erf(\frac{3\lambda\Delta x}{2})  \big)  } (\bar{u}_j+\bar{u}_{j+1}).
\end{align*}
To determine the shape parameter, we Taylor expand the right-hand side of the previous equation, which yields
\begin{align*}
    Au(x_{j+\frac{1}{2}}) &\approx \left(\frac{1}{2} +\frac{\lambda^2\Delta x^2 }{6} - \frac{7\lambda^4\Delta x^4}{90}\right)(\bar{u}_j+\bar{u}_{j+1}) \\
&= u(x_{j+\frac{1}{2}}) + {\Delta x^2}\Bigg(\frac{1}{3} {\lambda^2}u(x_{j+\frac{1}{2}}) + \frac1 6 u''(x_{j+\frac{1}{2}}) \Bigg) + \mathcal{O}(\Delta x^4).
\end{align*}
Hence, we have a second order approximation for the cell boundary point. Notice that we can obtain a fourth order approximation if we choose the shape parameter with
\begin{align*}
   {\lambda^2}=-\frac{u''(x_{j+\frac{1}{2}})}{2u(x_{j+\frac{1}{2}})}+\mathcal{O}(\Delta x^2).
\end{align*}
In practice, this ratio can be formed using the available cell average data. Derivatives in these expressions are approximated using finite differences, although there may be many ways to approximate these terms. Note that the data can be shifted by some positive constant at the beginning and end of the reconstruction steps to prevent division by zero, if needed. Lastly, if $\lambda^2$ is too large, we replace it with a constant whose sign matches $\lambda^2$ -- the particular value of this constant is not important. In the next section, we perform a similar reconstruction using a primitive function.


\subsubsection{Construction with a Primitive Function}
\label{subsubsec: A primitive function}

To reconstruct the approximation at the cell boundary $x=x_{j+\frac{1}{2}}$ from the cell averages $\{\bar{u}_j,\bar{u}_{j+1}\}$, we define a primitive function $$U(x)=\int_{x_{j-\frac{1}{2}}}^x u(\xi) d\xi$$ which can be explicitly written in terms of the available cell averages as 
$$U(x_{i-\frac{1}{2}})= \Delta x \sum_{\ell =j}^{i-1} \bar{u}_{\ell} \quad \text{ for } i=j,\cdots,j+2.$$
Using the available interpolatory data for the primitive function at the cell interfaces, we seek an RBF representation 
\begin{align}\label{rbf_app1}
AU(x):= \sum_{k=0}^{2} \alpha_k \phi \left(x-x_{j+k-\frac{1}{2}}\right),
\end{align}
which satisfies
\begin{align}\label{rbf_app1_cond}
    AU(x_{i-\frac{1}{2}})=U(x_{i-\frac{1}{2}}), \quad i=j,\cdots,j+2.
\end{align}
Then the final approximation to $u(x)$ at $x=x_{j+\frac{1}{2}}$ is obtained by differentiating the RBF representation
$$AU'(x):= \sum_{k=0}^{2} \alpha_k \phi'(x-x_{j+k-\frac{1}{2}}),$$ which approximates $U'(x)=u(x)$, i.e., 
\begin{align}\label{rbf_app1_fin0}
    AU'(x_{j+\frac{1}{2}}) \approx U'(x_{j+\frac{1}{2}})=u(x_{j+\frac{1}{2}}).
\end{align}
The approximation with a Gaussian RBF $\phi(x)$ is found to be
\begin{align}\label{eq:rbf_loc}
    AU'(x_{j+\frac{1}{2}})=2{\lambda^2}\Delta x^2\frac{ e^{3{\lambda^2}\Delta x^2} }{ e^{4{\lambda^2}\Delta x^2}-1}(\bar{u}_j+\bar{u}_{j+1}),
\end{align}
with the basis coefficients calculated from \eqref{rbf_app1_cond} and \eqref{rbf_app1_fin0}.
Applying a Taylor expansion to the right-hand side of this equation gives 
\begin{align*}
    AU'(x_{j+\frac{1}{2}}) &\approx \left(\frac{1}{2} +\frac{1}{2}\lambda^2\Delta x^2 - \frac{1}{12}{\lambda^4\Delta x^4}\right)(\bar{u}_j+\bar{u}_{j+1}) \\
&=u(x_{j+\frac{1}{2}}) + \Delta x^2 \Bigg({\lambda^2} u(x_{j+\frac{1}{2}})+\frac1 6 u''(x_{j+\frac{1}{2}})\Bigg) + \mathcal{O}(\Delta x^4).
\end{align*}
Hence, we have the second order approximation for the reconstructed cell boundary point. Alternatively, we can obtain the fourth order approximation if we choose the shape parameter with
\begin{align}\label{lam:local}
   {\lambda^2}=-\frac{u''(x_{j+\frac{1}{2}})}{6u(x_{j+\frac{1}{2}})}+\mathcal{O}(\Delta x^2),
\end{align}
which can be computed using the techniques previously described at the end of section \ref{subsubsec: Direct with integrals}.

Similarly, we can compute for the case of $N=4$. Using the cell averages $\{\bar{u}_{j}:j=-1,\cdots,2\}$, the approximation is defined by
\begin{align}\label{rbf_app1_4}
AU(x):= \sum_{k=-1}^{3} \alpha_k \phi(x-x_{j+k-\frac{1}{2}})
\end{align}
and at the cell boundary $x=x_{j+\frac{1}{2}}$, we have that
\begin{align}\label{rbf_app1_4_cond}
\begin{split}
    AU(x_{i-\frac{1}{2}})&=U(x_{i-\frac{1}{2}})\\ 
    &= \Delta x \sum_{\ell =j}^{i-1} \bar{u}_{\ell} 
    , \quad i=j-1,\cdots,j+3.
\end{split}
\end{align}

Proceeding as before, we can obtain the solution 
\begin{align}\label{eq:rbf_global}
     AU'(x_{j+\frac{1}{2}}) &\approx \sum_{k=-1}^{2} C_k \bar{u}_{j+k} 
\end{align}
with coefficients $C_k$ computed from equations \eqref{rbf_app1_4} and \eqref{rbf_app1_4_cond}. As before, these
can be Taylor expanded about the cell boundary $x=x_{j+\frac{1}{2}}$ and we find that
\begin{align*}
    AU'(x_{j+\frac{1}{2}})
    &= u(x_{j+\frac{1}{2}}) + {\Delta x^4}\left(\frac{1}{30}u^{(4)}(x_{j+\frac{1}{2}}) +  \frac23{\lambda^2}u''(x_{j+\frac{1}{2}}) + 2 u(x_{j+\frac{1}{2}}){\lambda^4} \right) + \mathcal{O}(\Delta x^6).
\end{align*}
Next, we choose $\lambda$ to remove the  $\mathcal{O}(\Delta x^4)$ term, i.e.,
\begin{align}\label{lam_choice}
    \lambda^2=\frac { -\frac{1}{3}u''(x_{j+\frac{1}{2}}) \pm \sqrt{\frac1 9 u''(x_{j+\frac{1}{2}})^2 - \frac{1}{15} u(x_{j+\frac{1}{2}})u^{(4)}(x_{j+\frac{1}{2}})}  } {2u(x_{j+\frac{1}{2}})} +  \mathcal{O}(\Delta x^p),
\end{align}
which can be computed using the same techniques previously discussed. Therefore we can obtain a superconvergent scheme, which is $(4+p)$th order accurate with $p\leq 2$.

\begin{theorem}
	Let $u$ be a smooth function on $\Omega$ and $\phi$ is a smooth radial basis function. Given a set of reference points $\{x_k\in\Omega:k=1,\cdots,N\}$ for an even integer $N$, there exists a set of coefficients $\{\alpha_k :k=1,\cdots,N\}$ of the approximation
	\begin{align*}
	Au(x) = \sum_{k=1}^{N} \alpha_k \phi(x-x_k)
	\end{align*}
	to the function $u(x)$, which are constructed from cell averaged data $\{\bar{u}(x_j) : x_j \in \Omega\}$. Moreover, the resulting approximation is $(N+p)$th order accurate, with $0\leq p\leq 2$, i.e.,
	\begin{align*}
	Au(x)=u(x)+ \mathcal{O}(\Delta x^{N+p}),
	\end{align*}
	for $x\in\Omega$.
\end{theorem}
The proof of this theorem is inductive and is a relatively direct  construction, as in the cases provided above. In this paper, we only supply the proper shape parameters for the case where $N$ is even. However, note that the analysis can be applied to odd values of $N$, which is provided in appendix \ref{Appendix: Theorem notes}. We now proceed to the discussion of WENO schemes in section \ref{sec: WENO schemes}, making use of the superconvergent RBF approximations.
